Outflows from Short-Lived Neutron-Star Merger Remnants Can Produce a Blue Kilonova

We present a 3D general-relativistic magnetohydrodynamic simulation of a short-lived neutron star remnant formed in the aftermath of a binary neutron star merger. The simulation uses an M1 neutrino transport scheme to track neutrino-matter interactions and is well-suited to studying the resulting nucleosynthesis and kilonova emission. We find that the ejecta in our simulations under-produce $r$-process abundances beyond the second $r$-process peak. For sufficiently long-lived remnants, these outflows \textit{alone} can produce blue kilonovae, including the blue kilonova component observed for AT2017gfo.

==> ApJL HMNS/header.tex <==
% ======================================================================
% packages
% ======================================================================
% \usepackage{fullpage}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{braket}
\usepackage{amssymb}
\usepackage{color}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{latexsym}
\usepackage{listings}
\usepackage{mathrsfs}
% \usepackage{aas_macros}
\usepackage{letltxmacro}
\usepackage[normalem]{ulem}

\usepackage{subfigure}
% pdfpages doesn't work with revtex.
% see:
% https://tex.stackexchange.com/questions/266520/including-pdfpages-renders-rotated-revtex-4-1-pdflatex-output
%\usepackage{pdfpages}

\usepackage{verbatim}
\usepackage{tabularx}
\usepackage{ragged2e}
\usepackage{multirow}
\usepackage{amsbsy}

% \usepackage{savesym}
% \savesymbol{tablenum}
% \usepackage{siunitx}
% \restoresymbol{SIX}{tablenum}

\usepackage{numprint}
\usepackage{makecell}
% need to include unicode to get dashes to work...
\usepackage[utf8]{inputenc}

%\usepackage{authorblk}
% \usepackage[colorlinks,citecolor=blue]{hyperref}

% ======================================================================
% Macros Jonah Likes
% ======================================================================
\newcommand{\R}{\mathbb{R}}
\newcommand{\eval}{\biggr\rvert} %evaluated at
\newcommand{\N}{\mathbb{N}} % Integers
% vectors. Pick bold symbols or the vector arrow.
%\newcommand{\myvec}[1]{\vec{#1}} 
%\newcommand{\myvec}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\myvec}[1]{\pmb{\mathbf{#1}}}

% total derivatives 
\newcommand{\diff}[2]{\frac{d #1}{d #2}} 
\newcommand{\dd}[1]{\frac{d}{d #1}}
% second total derivatives
\newcommand{\ddII }[1]{\frac{\partial^2}{\partial #1^2}}
% partial derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} 
\newcommand{\pdd}[1]{\frac{\partial}{\partial #1}} 
% second partial derivatives
\newcommand{\ppdd}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\pdII}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pddII}[1]{\frac{\partial^2}{\partial #1^2}}

% fractions
\newcommand{\half}{\frac{1}{2}}

% braces
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\sqrbrace}[1]{\left[ #1 \right]}
\newcommand{\curlybrace}[1]{\left\{ #1 \right\}}
\newcommand{\inner}[1]{\paren{#1}}
\newcommand{\norm}[1]{\left| #1 \right|_2}
\newcommand{\dwmean}[1]{\left\langle #1 \right\rangle_{\rho,r,\theta,\phi}}
\newcommand{\dwstd}[1]{\text{std}\left( #1 \right)_{\rho,r,\theta,\phi}}

% fix braket
\renewcommand{\braket}[1]{\left\langle #1 \right\rangle}

% vandermonde matrix
\newcommand{\V}{\mathcal{V}}

% Filter matrix
\newcommand{\F}{\mathcal{F}}

% Dmodal matrix
\newcommand{\M}{\mathcal{M}}
% Dnodal matrix
\newcommand{\DN}{\mathcal{N}}

% interval
\newcommand{\I}{\mathcal{I}}

% lie derivative
\newcommand{\Lie}{\mathcal{L}}

% asymptotic order
\newcommand{\Ord}[1]{\mathcal{O}\paren{#1}}

% fancy T
\newcommand{\mT}{\mathcal{T}}

% fancy I
\newcommand{\mI}{\mathcal{I}}

% stiffness
\newcommand{\St}{\mathcal{S}}

% error
\newcommand{\ME}{\mathcal{E}}

% energy norm
\newcommand{\MH}{\mathcal{H}}

% number of flops, memory domains
\newcommand{\NF}{\text{NF}}
\newcommand{\ND}{\text{ND}}
\newcommand{\OH}{\text{OH}}
\newcommand{\CO}{\text{CO}}
\newcommand{\MO}{\text{MO}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}

% FD and DG
\newcommand{\FD}{\text{FD}}
\newcommand{\DG}{\text{DG}}

% BSSN
\newcommand{\BSSN}{\text{BSSN}}

% bytes
\newcommand{\B}{\text{B}}

% (non)linear operator
\newcommand{\Lo}{\mathcal{L}}

% blight
\newcommand{\bhlight}{$\texttt{bhlight}$${}$}
\newcommand{\nubhlight}{$\nu\texttt{bhlight}$${}$}
\newcommand{\grmonty}{$\texttt{grmonty}$${}$}
\newcommand{\fornax}{$\texttt{FORNAX}$${}$}

% g
\newcommand{\detg}{\sqrt{-g}}

% neutrinos
\newcommand{\eepsilon}{\epsilon} % energy
\newcommand{\fin}{f\in \{\nu_e,\nu_{\bar{e}},\nu_x\}}
\newcommand{\sign}{\text{sign}(f)}
\newcommand{\jnuf}{j_{\eepsilon,f}}
\newcommand{\etanuf}{\eta_{\eepsilon,f}}
\newcommand{\Inuf}{I_{\eepsilon,f}}
\newcommand{\chinuf}{\chi_{\eepsilon,f}}
\newcommand{\sigmanuf}{\sigma_{\eepsilon,f}}
\newcommand{\alphanuf}{\alpha_{\eepsilon,f}}
\newcommand{\numin}{\nu_{\text{min}}}
\newcommand{\numax}{\nu_{\text{max}}}

% floors
\newcommand{\rhoflr}{\rho_{\text{flr}}}
\newcommand{\uflr}{u_{\text{flr}}}

% eos
\newcommand{\lT}{\log_{10}{T}}
\newcommand{\lrho}{\log_{10}{\rho}}
\newcommand{\lrhomin}{\log{\rho}_{\text{min}}}
\newcommand{\lTmin}{\log{T}_{\text{min}}}
\newcommand{\yemin}{(Y_e)_{\text{min}}}
\newcommand{\yemax}{(Y_e)_{\text{max}}}

% disk stuff
\newcommand{\Rin}{R_{\text{in}}}
\newcommand{\Rmax}{R_{\text{max}}}

% todo
\newcommand{\TODO}[1]{\textbf{[}{\color{red}TODO: }{\color{blue}#1}\textbf{]}}
\newcommand{\citeme}{\TODO{CITEME}}
\newcommand{\lookhere}[2]{\textbf{[}{\color{red}#1: }{\color{blue}#2}\textbf{]}}

% numprint setting
\npdecimalsign{.}
\npthousandsep{,}

% magic that allows for un-hyphenated right columns
\newcolumntype{Y}{>{\RaggedRight\arraybackslash}X}

% sets the path of graphics to be ./figures
% so includegraphics doesn't need "figures" to find stuff
\graphicspath{{./figures/}}

\frenchspacing
\sloppypar

